Feedback vertex sets of planar digraphs with fixed digirth

Let $fvs(G)$ denote the size of a minimum feedback vertex set of a digraph $G$. We study $fvs_g(n)$, which is the maximum $fvs(G)$ over all $n$-vertex planar digraphs $G$ of digirth $g$. We prove a planar-digraph analogue of the celebrated Lucchesi-Younger theorem showing that the minimum feedback vertex set is at most the maximum packing of a special type of directed cycles. As a corollary, we derive that $fvs_g(n)\le \frac{n-2}{g-2}$ for all $g\geq 3$. This improves all previously known upper bounds for $g \ge 4$, and for $g \ge 6$ it supersedes the best known upper bound of $\frac{2n-6}{g}$ (Esperet, Lemoine and Maffray, 2017) by a factor of 2. On the other hand, we develop a new framework to construct planar digraphs of fixed digirth and large $fvs$. Using it, for $g = 6$ and every $g \ge 8$, we construct an infinite family of planar digraphs of digirth $g$ and $fvs(G) = \frac{g+2}{g^2} n + O(1)$. For $g= 7$, our construction gives $fvs(G) = \frac{2}{11} n + O(1)$ and for $g = 4$ and $5$, $fvs(G) = \frac{n}{g-1}$. These improve the best known lower bound of $\frac{n-1}{g-1}$ (Knauer, Valicov and Wenger, 2017) for all $g \ge 4$. We thus obtain the two-sided bound $\frac{g+2}{g^2} \le \sup_{n \ge 1} \frac{fvs_g(n)}{n} \le \frac{1}{g-2}$ for all values $g = 6$ and every $g \ge 8$. The gap between the lower and the upper bound for $\sup_{n \ge 1} \frac{fvs_g(n)}{n}$ decreases from $\frac{g-2}{g(g-1)}$ to $\frac{4}{g^2(g-2)}$.

==> preamble.tex <==
\ProvidesFile{preamble.tex}


% Packages -----------------------------------------------------------------------------------------------
\usepackage[T1]{fontenc}
\usepackage{lmodern}
\usepackage[table]{xcolor}
\usepackage{stmaryrd}
\usepackage{bbold}
\usepackage{multirow}



% Packages du template de base ----------------------------------------------------------------
\usepackage{microtype}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{caption}
\captionsetup{belowskip=0pt,aboveskip=0pt}
\usepackage{subcaption}

\usepackage{graphicx}
\usepackage{amsthm}
\usepackage{thmtools}
\usepackage{float}
\usepackage[shortlabels]{enumitem}
\usepackage{hyperref,cleveref,cite,url}
\hypersetup{
 colorlinks,
 citecolor=green!50!black,
 linkcolor=red,
 urlcolor=blue!50!black}

\usepackage{pgf,tikz}

\usepackage{tkz-graph}
\usetikzlibrary{arrows.meta,decorations.markings,bbox,snakes,shapes.misc}


\tikzset{
  decoration={snake},
  cross/.style={cross out, draw=black, minimum size=2*(#1-\pgflinewidth), inner sep=0pt, outer sep=0pt},
  ->-/.style={decoration={
      markings,
      mark=at position #1 with {\arrow{>}}
    },postaction={decorate}},
  ->-/.default=0.55 % default position for the arrow on edges
}

\usetikzlibrary{automata}
\usetikzlibrary{patterns}

\usetikzlibrary{backgrounds,calc,positioning}
\usepackage{authblk}







% Numerotation des sections et indentation --------------------------------------------------------------

\parindent 0mm
\parskip 3mm

\setenumerate{label=\textup{(\arabic*)}, noitemsep, topsep=-\parskip, labelindent=.2em, leftmargin=*}
\setitemize{noitemsep, topsep=-\parskip, labelindent=.2em, leftmargin=*}



\setlist[itemize]{label=$\bullet$}


\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{observation}[theorem]{Observation}
\newtheorem*{observation*}{Observation}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{claim}[theorem]{Claim}
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{remark*}{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{application}[theorem]{Application}
\crefname{conjecture}{Conjecture}{Conjectures}




\newenvironment{reptheorem}[1]{%
 \renewcommand{\thetheorem}{\ref{#1}}
 \begin{theorem}}%
 {\end{theorem}
 \addtocounter{theorem}{-1}
 \renewcommand{\thetheorem}{\arabic{theorem}}}
 
  \newenvironment{replemma}[1]{%
 \renewcommand{\thelemma}{\ref{#1}}
 \begin{lemma}}%
 {\end{lemma}
 \addtocounter{lemma}{-1}
 \renewcommand{\thelemma}{\arabic{lemma}}}



\newcommand{\NN}[0]{\mathbb{N}}
\newcommand{\IntSet}[2]{\left \llbracket #1 ; #2 \right \rrbracket}
\newcommand{\Modul}[1]{\left | #1 \right |}
\newcommand{\Ent}[1]{\left \lfloor #1 \right \rfloor}
\newcommand{\Set}[2]{\left \lbrace #1 \; | \; #2 \right \rbrace}
\DeclareMathOperator{\mult}{mult}
\newcommand{\fa}{fas}
\newcommand{\fv}{fvs}

\DeclareMathOperator{\Root}{Root}
\DeclareMathOperator{\Ch}{Ch}

\renewcommand{\deg}{d}
\newcommand{\degout}{d^{+}}
\newcommand{\degin}{d^{-}}

\makeatletter
\newcommand{\segmentval}[2]{%
  \@ifnextchar\bgroup
    {\segmentval@witharg{#1}{#2}}
    {\delta_{#1}^{#2}}%
}
\newcommand{\segmentval@witharg}[3]{\delta_{#1}^{#2}(#3)}
\makeatother

